Probabilistic Gradient-Based Extrema Tracking

Feature tracking is a common task in visualization applications, where methods based on topological data analysis (TDA) have successfully been applied in the past for feature definition as well as tracking. In this work, we focus on tracking extrema of temporal scalar fields. A family of TDA approaches address this task by establishing one-to-one correspondences between extrema based on discrete gradient vector fields. More specifically, two extrema of subsequent time steps are matched if they fall into their respective ascending and descending manifolds. However, due to this one-to-one assignment, these approaches are prone to fail where, e.g., extrema are located in regions with low gradient magnitude, or are located close to boundaries of the manifolds. Therefore, we propose a probabilistic matching that captures a larger set of possible correspondences via neighborhood sampling, or by computing the overlap of the manifolds. We illustrate the usefulness of the approach with two application cases.

==> Figures/electronic_density/graph.tex <==
\begin{tikzpicture}[scale=1]
    % timestep lines
    \foreach \x [evaluate=\x as \xpos using 4.95 * (\x - 40)/30 -2.475] in {40, 45,  ..., 70}{
        \draw[gray, line width=0.05mm] (\xpos, -1.85) -- (\xpos, 1.85);
    }

    % graph
    \node(graph) at (0,0) {
        \includegraphics[width=5cm]{./Figures/electronic_density/FullTrackingGraph-fig.png}
    };
    
    % timestep labels
    \foreach \x [evaluate=\x as \xpos using 5 * (\x - 40)/30 -2.5] in {40, 45,  ..., 70}{
        \node[scale=0.75] at (\xpos, -2) {\tiny \x};
    }
    \node at (0, -2.25) {\tiny Timestep ($t$) $\rightarrow$};

    %timestep closeup
    \foreach \x [evaluate=\x as \xpos using 1.875 * (\x - 51)/6 + 2.85] in {51, 52, ..., 57}{
        \node[scale=0.75] at (\xpos, 0) {\tiny \x};
        \draw[gray, line width=0.01mm] (\xpos, 0.25) -- (\xpos, 1.55);
        \draw[gray, line width=0.01mm] (\xpos + 0.02, -1.575) -- (\xpos + 0.02, -0.25);
    }


   % closeup image one - to -one
    \node[draw=black, line width=0.5pt, inner sep=1pt](closeup) [ above right =0.1 mm and 0.1mm of graph.5] {
        \includegraphics[width=2.25 cm]{./Figures/electronic_density/closeup-onecoding}
    };

    % closeup image manifold overlapp
    \node[draw=black, line width=0.5pt, inner sep=1pt](manifold) [ below right =0.1 mm and 0.1mm of graph.355] {
        \includegraphics[width=2.25cm]{./Figures/electronic_density/closeup-manifold}
    };

    % colormap one-to-one
    \node[inner ysep= 0pt] (colormap-one)[right= 0.1mm of closeup] {
        \includegraphics[height=1.25cm]{./Figures/electronic_density/Colormap-Onetoone}
    };
    \node[align=center] [right= 0.01mm of colormap-one.70] {\tiny Bidirectional};
    \node[align=center] [right= 0.01mm of colormap-one.0] {\tiny Forward};
    \node[align=center] [right= 0.01mm of colormap-one.290] {\tiny Backward};

    % color map manifold
    \node[inner ysep= 0pt] (colormap-mf)[right= 0.1mm of manifold] {
        \includegraphics[height=1.25cm]{./Figures/electronic_density/Colormap-Manifold}
    };
    \node [below= 0.001mm of colormap-mf.290] {\tiny 0};
    \node [above = 0.001mm of colormap-mf.70] {\tiny 1};
    \node[align=center] [right= 0.01mm of colormap-mf] {\tiny Maximum manifold\\[-1.5ex]\tiny overlap};

    % timestep


    % EMBEDDINGS
    \node[draw=gray, inner sep=0pt](t51) at (-1.5,3) {
        \includegraphics[width=2cm]{./Figures/electronic_density/closeup-embedding-t51}
    };
    \node[draw=gray, inner sep=0pt](t53) at (0.75,3) {
        \includegraphics[width=2cm]{./Figures/electronic_density/closeup-embedding-t53}
    };
    \node[draw=gray, inner sep=0pt](t55) at (3,3) {
        \includegraphics[width=2cm]{./Figures/electronic_density/closeup-embedding-t55}
    };
    \node[draw=gray, inner sep=0pt](t65) at (5.25,3) {
        \includegraphics[width=2cm]{./Figures/electronic_density/closeup-embedding-t65}
    };

    % EMBEDDINGS labels
    \node[scale=0.75, below = 0.01mm of t51] {\tiny $t=$51};
    \node[scale=0.75, below = 0.01mm of t53] {\tiny $t=$53};
    \node[scale=0.75, below = 0.01mm of t55] {\tiny $t=$55};
    \node[scale=0.75, below = 0.01mm of t65] {\tiny $t=$65};
    
    
\end{tikzpicture}%

==> Figures/illustrations/correspondence/matrix-ex.tex <==
\begin{tikzpicture}[xscale=\scaleX,yscale=\scaleY]

  % CONTINUATION
  \begin{scope}[xshift=0,yshift=1.4cm, opacity=0.5]
    \matrix (features_t) [matrix of nodes,row sep=-\pgflinewidth,nodes={matrixCell}, ] {
      x & y & z & w \\
    };
  \end{scope}
  \begin{scope}[xshift=-2.55cm,yshift=0, opacity=0.5]
    \matrix (features_t_1) [matrix of nodes,row sep=-\pgflinewidth,nodes={matrixCell}]{
      a \\
      b \\
      c \\
      d \\
    };
  \end{scope}
  \begin{scope}[xshift=0,yshift=0]
    \matrix [matrix of nodes,row sep=-\pgflinewidth,nodes={matrixCell}]{
      0.90 & 0.10 & 0.00 & 0.00 \\
      0.00 & 0.90 & 0.00 & 0.00 \\
      0.00 & 0.00 & 0.32 & 0.55 \\
      0.00 & 0.00 & 0.00 & 0.76 \\
    };
  \end{scope}

  \node[] (top_time) [above = 0.01mm of features_t] {\textbf{t}};
  \node[] (left_time) [left = 0.01mm of features_t_1] {\textbf{t-1}};

  
\end{tikzpicture}

==> sections/algorithmFigure.tex <==
\usetikzlibrary{shadows,shadows.blur,arrows,positioning}
% Define the layers to draw the diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\definecolor{csGreen}{RGB}{127,205,187}
\definecolor{csBlue}{RGB}{44,127,184}

% Define block styles
\tikzstyle{materia}=[draw, fill=csBlue!20, text width=6.0em, text centered,
  minimum height=1.5em]
\tikzstyle{etape} = [materia, text width=16em, minimum width=10em,
  minimum height=3em, rounded corners, blur shadow={
    shadow blur steps=10,
    shadow blur extra rounding=2pt
  }]
\tikzstyle{texto} = [above, text width=6em, text centered]
\tikzstyle{linepart} = [draw, thick, color=black!50, -latex', dashed]
\tikzstyle{line} = [draw, thick, color=black!60, -latex']
\tikzstyle{ur}=[draw, text centered, minimum height=0.01em]

% Define distances for bordering
\newcommand{\blockdist}{1.3}
\newcommand{\edgedist}{1.5}

\newcommand{\etape}[2]{node (p#1) [etape]
  {#2}}

% Draw background
\newcommand{\background}[5]{%
  \begin{pgfonlayer}{background}
    % Left-top corner of the background rectangle
    \path (#1.west |- #2.north)+(-0.5,0.25) node (a1) {};
    % Right-bottom corner of the background rectangle
    \path (#3.east |- #4.south)+(+0.5,-0.25) node (a2) {};
    % Draw the background
    % \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
    %   (a1) rectangle (a2);
    %   \path (#3.east |- #2.north)+(0,0.25)--(#1.west |- #2.north) node[midway] (#5-n) {};
    %   \path (#3.east |- #2.south)+(0,-0.35)--(#1.west |- #2.south) node[midway] (#5-s) {};
    %   \path (#3.east |- #2.north)+(0.7,0)--(#3.east |- #4.south) node[midway] (#5-w) {};
  \end{pgfonlayer}}

\newcommand{\transreceptor}[3]{%
  \path [linepart] (#1.east) -- node [above]
    {\scriptsize #2} (#3);}

\begin{figure}[tbh]
    \begin{center}
        \begin{tikzpicture}[scale=0.8,transform shape]
            % Draw diagram elements
            \path \etape{1}{Initialization};

            \path (p1.south)+(0.0,-1.0) \etape{2}{CP Tracking};
            \path (p2.south)+(0.0,-1.5) \etape{3}{Basic Filtering};
            \path (p3.south)+(0.0,-1.0) \etape{4}{Generation of Hierarchical Features};
            \path (p4.south)+(0.0,-1.0) \etape{5}{Extraction of Feature Tracks};
            \path (p5.south)+(0.0,-1.0) \etape{6}{Visualization};

            \coordinate[left of=p2] (r0);
            %\coordinate[left of=p7] (r1);

            % Draw arrows between elements
            \path [line] (p1.south) -- node [above] {} (p2);
            \path [line] (p2.south) -- node [anchor=west] {Raw Tracking Graph} (p3);
            \path [line] (p3.south) -- node [above] {} (p4);
            \path [line] (p4.south) -- node [above] {} (p5);
            \path [line] (p5.south) -- node [above] {} (p6);

            % \path [line] (p7.west) -- node [above] {loop} ([xshift=-3.25cm]r1) -- ([xshift=-3.25cm]r0) -- (p2.west);

            \background{p5}{p5}{p6}{p6}{bk1}

        \end{tikzpicture}
    \end{center}
    \caption{\textbf{Algorithm:} Our algorithm is based on six main building blocks. This modular approach allows for high flexibility and allows domain specific customization and future extension.}
    \label{fig:algorithm1}
\end{figure}
